Parallelism and Time in Hierarchical Self-Assembly

We study the role that parallelism plays in time complexity of Winfree's abstract Tile Assembly Model (aTAM), a model of molecular algorithmic self-assembly. In the "hierarchical" aTAM, two assemblies, both consisting of multiple tiles, are allowed to aggregate together, whereas in the "seeded" aTAM, tiles attach one at a time to a growing assembly. Adleman, Cheng, Goel, and Huang ("Running Time and Program Size for Self-Assembled Squares", STOC 2001) showed how to assemble an n x n square in O(n) time in the seeded aTAM using O(log n / log log n) unique tile types, where both of these parameters are optimal. They asked whether the hierarchical aTAM could allow a tile system to use the ability to form large assemblies in parallel before they attach to break the Omega(n) lower bound for assembly time. We show that there is a tile system with the optimal O(log n / log log n) tile types that assembles an n x n square using O(log^2 n) parallel "stages", which is close to the optimal Omega(log n) stages, forming the final n x n square from four n/2 x n/2 squares, which are themselves recursively formed from n/4 x n/4 squares, etc. However, despite this nearly maximal parallelism, the system requires superlinear time to assemble the square. We extend the definition of *partial order tile systems* studied by Adleman et al. in a natural way to hierarchical assembly and show that no hierarchical partial order tile system can build any shape with diameter N in less than time Omega(N), demonstrating that in this case the hierarchical model affords no speedup whatsoever over the seeded model. We strengthen the Omega(N) time lower bound for deterministic seeded systems of Adleman et al. to nondeterministic seeded systems. Finally, we show that for infinitely many n, a tile system can assemble an n x n' rectangle, with n > n', in time O(n^{4/5} log n), breaking the linear-time lower bound.

==> hierarchical.tex <==
\section{Hierarchical Self-Assembly: Parallelism and Time}
\label{sec-hierarchical}


\opt{normal}{
    In this section we show that under the hierarchical model of tile assembly, it is possible to self-assemble an $n \times n$ square, for arbitrary $n \in \Z^+$, using the asymptotically optimal $O(\frac{\log n}{\log \log n})$ number of tile types.
    Furthermore, the square assembles using nearly the maximum possible parallelism in the hierarchical model, building the final square out of four assembled sub-squares of size $n/2 \times n/2$, which are themselves each assembled from four sub-squares of size $n/4 \times n/4$, etc.
    The sub-optimality stems from the need for us to construct the smallest sub-squares of size $O(\log n) \times O(\log n) = O(\log^2 n)$ without parallelism.
    
    We then show the somewhat counterintuitive result that this construction is \emph{slower} than the construction of~\cite{AdChGoHu01}, which assembles an $n \times n$ square in time $O(n)$ in the seeded aTAM.
    The authors of \cite{AdChGoHu01} define a class of seeded TAS's called \emph{partial order systems}, whose definition we extend in a natural way to hierarchical systems.
    We show, using basic principles of chemical kinetics, that \emph{no} partial order system can assemble any shape of size $N$ in faster than $\Omega(\sqrt{N})$ time.
    Thus hierarchical partial order systems achieve no speedup at all over seeded systems.
    Finally, we show that by breaking the partial order assumption, it is possible to assemble a rectangle in time sublinear in its diameter.
    %This implies that among partial order systems, the TAS described in~\cite{AdChGoHu01} for assembling an $n \times n$ square is in fact optimal, in both tile complexity and in assembly time, for the hierarchical model as well.
    %We note, however, that there are other theoretical advantages to the hierarchical model, for instance, the use of steric hindrance to enable algorithmic fault-tolerance~\cite{DotPatReiSchSum10}.
}


\input{two-handed-square}
\input{two-handed-assembly-time}
\input{lower-bound}
\input{fast-rectangle}


==> tam.tex <==
\section{Abstract Tile Assembly Model}
\label{sec-tam-informal}

\newcommand{\fullgridgraph}{G^\mathrm{f}}
\newcommand{\bindinggraph}{G^\mathrm{b}}

This section gives a terse definition of the abstract Tile Assembly Model (aTAM,~\cite{Winf98}). This is not a tutorial; for readers unfamiliar with the aTAM,  \cite{RotWin00} gives an excellent introduction to the model.

Fix an alphabet $\Sigma$. $\Sigma^*$ is the set of finite strings over $\Sigma$.
Given a discrete object $O$, $\langle O \rangle$ denotes a standard encoding of $O$ as an element of $\Sigma^*$.
$\Z$, $\Z^+$, $\N$, $\R^+$ denote the set of integers, positive integers, nonnegative integers, and nonnegative real numbers, respectively.
For all $n \in \N$, $[n]$ denotes the set $\{0, 1, \ldots, n-1\}$.
For a set $A$, $\calP(A)$ denotes the power set of $A$.
Given $A \subseteq \Z^2$, the \emph{full grid graph} of $A$ is the undirected graph $\fullgridgraph_A=(V,E)$, where $V=A$, and for all $u,v\in V$, $\{u,v\} \in E \iff \| u-v\|_2 = 1$; i.e., iff $u$ and $v$ are adjacent on the integer Cartesian plane.
A \emph{shape} is a set $S \subseteq \Z^2$ such that $\fullgridgraph_S$ is connected.
%A shape $S$ is a \emph{tree} if $\fullgridgraph_S$ is acyclic.


A \emph{tile type} is a tuple $t \in (\Sigma^*)^4$; i.e., a unit square with four sides listed in some standardized order, each side having a \emph{glue label} (a.k.a. \emph{glue}) $\ell \in \Sigma^*$.
%consisting of a finite string \emph{label} and nonnegative integer \emph{strength}.
For a set of tile types $T$, let $\Lambda(T)$ denote the set of all glue labels of tile types in $T$.
We assume a finite set $T$ of tile types, but an infinite number of copies of each tile type, each copy referred to as a \emph{tile}. An \emph{assembly}
is a nonempty connected arrangement of tiles on the integer lattice $\Z^2$, i.e., a partial function $\alpha:\Z^2 \dashrightarrow T$ such that $\fullgridgraph_{\dom \alpha}$ is connected and $\dom \alpha \neq \emptyset$. The \emph{shape of $\alpha$} is $\dom \alpha$.
A \emph{strength function} is a function $g:\Lambda(T)\to\N$ indicating, for each glue label $\ell$, the strength $g(\ell)$ with which it binds.
Two adjacent tiles in an assembly \emph{interact} if the glue labels on their abutting sides are equal and have positive strength according to $g$.
Each assembly $\alpha$ induces a \emph{binding graph} $\bindinggraph_\alpha$, a grid graph whose vertices are positions occupied by tiles, with an edge between two vertices if the tiles at those vertices interact.\footnote{For $\fullgridgraph_{\dom \alpha}=(V_{\dom \alpha},E_{\dom \alpha})$ and $\bindinggraph_\alpha=(V_\alpha,E_\alpha)$, $\bindinggraph_\alpha$ is a spanning subgraph of $\fullgridgraph_{\dom \alpha}$: $V_\alpha = V_{\dom \alpha}$ and $E_\alpha \subseteq E_{\dom \alpha}$.}
Given $\tau\in\Z^+$, $\alpha$ is \emph{$\tau$-stable} if every cut of $\bindinggraph_\alpha$ has weight at least $\tau$, where the weight of an edge is the strength of the glue it represents.
That is, $\alpha$ is $\tau$-stable if at least energy $\tau$ is required to separate $\alpha$ into two parts.
When $\tau$ is clear from context, we say $\alpha$ is \emph{stable}.
Given two assemblies $\alpha,\beta:\Z^2 \dashrightarrow T$, we say $\alpha$ is a \emph{subassembly} of $\beta$, and we write $\alpha \sqsubseteq \beta$, if $\dom \alpha \subseteq \dom \beta$ and, for all points $p \in \dom \alpha$, $\alpha(p) = \beta(p)$.





\subsection{Seeded aTAM}
A \emph{seeded tile assembly system} (seeded TAS) is a triple $\calT = (T,\sigma,g,\tau)$, where $T$ is a finite set of tile types, $\sigma:\Z^2 \dashrightarrow T$ is the finite, $\tau$-stable \emph{seed assembly}, $g:\Lambda(T)\to\N$ is the \emph{strength function}, and $\tau\in\Z^+$ is the \emph{temperature}.
Given two $\tau$-stable assemblies $\alpha,\beta:\Z^2 \dashrightarrow T$, we write $\alpha \to_1^{\calT} \beta$ if $\alpha \sqsubseteq \beta$ and $|\dom \beta \setminus \dom \alpha| = 1$. In this case we say $\alpha$ \emph{$\calT$-produces $\beta$ in one step}.\footnote{Intuitively $\alpha \to_1^\calT \beta$ means that $\alpha$ can grow into $\beta$ by the addition of a single tile; the fact that we require both $\alpha$ and $\beta$ to be $\tau$-stable implies in particular that the new tile is able to bind to $\alpha$ with strength at least $\tau$. It is easy to check that had we instead required only $\alpha$ to be $\tau$-stable, and required that the cut of $\beta$ separating $\alpha$ from the new tile has strength at least $\tau$, then this implies that $\beta$ is also $\tau$-stable.}
If $\alpha \to_1^{\calT} \beta$, $ \dom \beta \setminus \dom \alpha=\{p\}$, and $t=\beta(p)$, we write $\beta = \alpha + (p \mapsto t)$.
The \emph{$\calT$-frontier} of $\alpha$ is the set $\partial^\calT \alpha = \bigcup_{\alpha \to_1^\calT \beta} \dom \beta \setminus \dom \alpha$, the set of empty locations at which a tile could stably attach to $\alpha$.
%The \emph{$t$-frontier} $\partial_t \alpha \subseteq \partial \alpha$ of $\alpha$ is the set $\setr{p\in\partial \alpha}{\alpha \to_1^\calT \beta \text{ and } \beta(p)=t}.$

A sequence of $k\in\Z^+ \cup \{\infty\}$ assemblies $\vec{\alpha} = (\alpha_0,\alpha_1,\ldots)$ is a \emph{$\calT$-assembly sequence} if, for all $1 \leq i < k$, $\alpha_{i-1} \to_1^\calT \alpha_{i}$.
We write $\alpha \to^\calT \beta$, and we say $\alpha$ \emph{$\calT$-produces} $\beta$ (in 0 or more steps) if there is a $\calT$-assembly sequence $\vec{\alpha}=(\alpha_0,\alpha_1,\ldots)$ of length $k = |\dom \beta \setminus \dom \alpha| + 1$ such that
1) $\alpha = \alpha_0$,
2) $\dom \beta = \bigcup_{0 \leq i < k} \dom {\alpha_i}$, and
3) for all $0 \leq i < k$, $\alpha_{i} \sqsubseteq \beta$.
In this case, we say that $\beta$ is the \emph{result} of $\vec{\alpha}$, written $\beta=\res{\vec{\alpha}}$.
If $k$ is finite then it is routine to verify that $\res{\vec{\alpha}} = \alpha_{k-1}$.\footnote{If we had defined the relation $\to^\calT$ based on only finite assembly sequences, then $\to^\calT$ would be simply the reflexive, transitive closure $(\to_1^\calT)^*$ of $\to_1^\calT$. But this would mean that no infinite assembly could be produced from a finite assembly, even though there is a well-defined, unique ``limit assembly'' of every infinite assembly sequence.} 
We say $\alpha$ is \emph{$\calT$-producible} if $\sigma \to^\calT \alpha$, and we write $\prodasm{\calT}$ to denote the set of $\calT$-producible assemblies.
The relation $\to^\calT$ is a partial order on $\prodasm{\calT}$ \cite{Roth01,jSSADST}.\footnote{In fact it is a partial order on the set of $\tau$-stable assemblies, including even those that are not $\calT$-producible.}
%Note that all $\calT$-producible assemblies are $\tau$-stable.
A $\calT$-assembly sequence $\alpha_0,\alpha_1,\ldots$ is \emph{fair} if, for all $i$ and all $p\in\partial^\calT\alpha_i$, there exists $j$ such that $\alpha_j(p)$ is defined; i.e., no frontier location is ``starved''.

\newcommand{\w}[1]{\widetilde{#1}}
\newcommand{\wa}{\w{\alpha}}
\newcommand{\wb}{\w{\beta}}
\newcommand{\wg}{\w{\gamma}}

%Given a TAS $\calT=(T,\sigma,\tau)$, an assembly $\alpha$ is \emph{$\calT$-producible}, or \emph{producible} if $\calT$ is clear from context, if either $\alpha = \sigma$, or $\alpha$ results from the $\tau$-stable attachment of a single tile to a producible assembly (``$\tau$-stable attachment'' meaning that the cut separating the tile from the rest of the assembly has strength $\geq \tau$, which implies by induction that $\alpha$ is $\tau$-stable).
An assembly $\alpha$ is \emph{$\calT$-terminal} if $\alpha$ is $\tau$-stable and $\partial^\calT \alpha=\emptyset$.
It is easy to check that an assembly sequence $\vec{\alpha}$ is fair if and only $\res{\vec{\alpha}}$ is terminal.
We write $\termasm{\calT} \subseteq \prodasm{\calT}$ to denote the set of $\calT$-producible, $\calT$-terminal assemblies.
Let $\alpha$ be an assembly, and let $\wa$ denote the set of all assemblies that are equivalent to $\alpha$ up to translation.
We have fixed assemblies at certain positions on $\Z^2$ only for mathematical convenience in some contexts, but of course real assemblies float freely in solution and do not have a fixed position.
For clarity we often abuse notation and take $\alpha$ to be the same object as $\wa$.

A seeded TAS $\calT$ is \emph{directed (a.k.a., deterministic, confluent)} if the poset $(\prodasm{\calT}, \to^\calT)$ is directed; i.e., if for each $\alpha,\beta \in \prodasm{\calT}$, there exists $\gamma\in\prodasm{\calT}$ such that $\alpha \to^\calT \gamma$ and $\beta \to^\calT \gamma$.\footnote{The following two convenient characterizations of ``directed'' are routine to verify.
%It is routine to verify that the following two convenient definitions of ``directed'' are equivalent to the stated definition.
$\calT$ is directed if and only if $|\termasm{\calT}| = 1$ (of course by this we mean that all the terminal assemblies are equivalent up to translation). $\calT$ is \emph{not} directed if and only if there exist $\alpha,\beta\in\prodasm{\calT}$ and $p \in \dom \alpha \cap \dom \beta$ such that $\alpha(p) \neq \beta(p)$.}
We say that a TAS $\calT$ \emph{strictly self-assembles} a shape $S \subseteq \Z^2$ if, for all $\alpha \in \termasm{\calT}$, $\dom \alpha = S$; i.e., if every terminal assembly produced by $\calT$ has shape $S$.
If $\calT$ strictly self-assembles some shape $S$, we say that $\calT$ is \emph{strict}.
Note that the implication ``$\calT$ is directed $\implies$ $\calT$ is strict'' holds, but the converse does not hold.


\subsection{Hierarchical aTAM}
A \emph{hierarchical tile assembly system} (hierarchical TAS) is a triple $\calT = (T,g,\tau)$, where $T$ is a finite set of tile types, $g:\Lambda(T)\to\N$ is the \emph{strength function}, and $\tau\in\Z^+$ is the \emph{temperature}.
Let $\alpha,\beta:\Z^2 \dashrightarrow T$ be two assemblies.
Say that $\alpha$ and $\beta$ are \emph{nonoverlapping} if $\dom\alpha \cap \dom\beta = \emptyset$.
If $\alpha$ and $\beta$ are nonoverlapping assemblies, define $\alpha \cup \beta$ to be the assembly $\gamma$ defined by $\gamma(p) = \alpha(p)$ for all $p\in\dom\alpha$, $\gamma(p) = \beta(p)$ for all $p \in \dom \beta$, and $\gamma(p)$ is undefined for all $p \in \Z^2 \setminus (\dom\alpha \cup \dom\beta)$.
An assembly $\gamma$ is \emph{singular} if $\gamma(p)=t$ for some $p\in\Z^2$ and some $t \in T$ and $\gamma(p')$ is undefined for all $p' \in \Z^2 \setminus \{p\}$.
Given a hierarchical TAS $\calT=(T,g,\tau)$, an assembly $\gamma$ is \emph{$\calT$-producible} if either 1) $\gamma$ is singular, or 2) there exist producible nonoverlapping assemblies $\alpha$ and $\beta$ such that $\gamma = \alpha\cup\beta$ and $\gamma$ is $\tau$-stable.\footnote{Unlike some definitions of the hierarchical aTAM, we have not allowed for translation of $\alpha$ and $\beta$ to determine whether they can stably attach.  This is because every translation of every producible assembly is itself producible.}
In the latter case, write $\alpha + \beta \to \gamma$.
An assembly $\alpha$ is \emph{$\calT$-terminal} if for every producible assembly $\beta$ such that $\alpha$ and $\beta$ are nonoverlapping, $\alpha \cup \beta$ is not $\tau$-stable.\footnote{The restriction on overlap is a model of a chemical phenomenon known as \emph{steric hindrance}~\cite[Section 5.11]{WadeOrganicChemistry91} or, particularly when employed as a design tool for intentional prevention of unwanted binding in synthesized molecules, \emph{steric protection}~\cite{HellerPugh1,HellerPugh2,GotEtAl00}.}
Define $\prodasm{\calT}$ to be the set of all $\calT$-producible assemblies.
Define $\termasm{\calT} \subseteq \prodasm{\calT}$ to be the set of all $\calT$-producible, $\calT$-terminal assemblies.
A hierarchical TAS $\calT$ is \emph{directed (a.k.a., deterministic, confluent)} if $|\termasm{\calT}|=1$.\footnote{Again, technically by this we mean that the quotient set of $\termasm{\calT}$ under the equivalence relation defined by equality under translation is a singleton set.}
We say that a TAS $\calT$ \emph{strictly self-assembles} a shape $S \subseteq \Z^2$ if, for all $\alpha \in \termasm{\calT}$, $\dom \alpha = S$; i.e., if every terminal assembly produced by $\calT$ has shape $S$.

Let $\calT$ be a hierarchical TAS, and let $\alpha \in \prodasm{\calT}$ be a $\calT$-producible assembly.
An \emph{assembly tree} $\Upsilon$ of $\widehat{\alpha}$ is a full binary tree with $|\dom\widehat{\alpha}|$ leaves, whose nodes are labeled by $\calT$-producible assemblies, with $\widehat{\alpha}$ labeling the root, singular assemblies labeling the leaves, and node $u$ labeled with $\gamma$ having children $u_1$ labeled with $\alpha$ and $u_2$ labeled with $\beta$, with the requirement that $\alpha + \beta \to \gamma$.
That is, $\Upsilon$ represents one possible pathway through which $\widehat{\alpha}$ could be produced from individual tile types in $\calT$.
Let $\Upsilon(\calT)$ denote the set of all assembly trees of $\calT$.
Say that an assembly tree is \emph{$\calT$-terminal} if its root is a $\calT$-terminal assembly.
Let $\Upsilon_\Box(\calT)$ denote the set of all $\calT$-terminal assembly trees of $\calT$.
Note that even a directed hierarchical TAS can have multiple terminal assembly trees that all have the same root terminal assembly.




%In this paper we will always use \emph{singly-seeded temperature-2} TAS's, those with $|\dom \sigma|=1$ and $\tau=2$; hence we will use the term \emph{seed tile} for $\sigma$ as well, and for the remainder of this paper we use the term TAS to mean singly-seeded temperature-2 TAS.
When $\calT$ is clear from context, we may omit $\calT$ from the notation above and instead write
$\to_1$,
$\to$,
$\partial \alpha$,
\emph{frontier},
\emph{assembly sequence},
\emph{produces},
\emph{producible}, and
\emph{terminal}.
%Since the behavior of a TAS $\calT=(T,\sigma,2)$ is unchanged if every glue with strength greater than 2 is changed to have strength exactly 2, we assume henceforth that all glue strengths are 0, 1, or 2, and use the terms \emph{null glue}, \emph{single glue}, and \emph{double glue}, respectively, to refer to these three cases.\footnote{We use \emph{null bond}, \emph{single bond}, and \emph{double bond} similarly to refer to the \emph{interaction} of two tiles.}
We also assume without loss of generality that every single glue or double glue occurring in some tile type in some direction also occurs in some tile type in the opposite direction, i.e., there are no ``effectively null'' single or double glues.
%\footnote{Thus the existence of a tile with a double glue facing empty space implies that the empty space is part of the frontier. Many of our arguments use the contrapositive that if a shape $S$ is strictly self-assembled by a tile assembly system and a side of a tile faces a point $p \not\in S$, then the tile cannot have a double glue on that side.}




==> two-handed-assembly-time.tex <==
\section{Time Complexity in the Hierarchical Model}
\label{sec-runtime}

In this section we define a formal notion of time complexity for hierarchical tile assembly systems. %, in order to show that the subset of systems known as partial order systems cannot assemble any shape of $L_1$ diameter $N$ in faster than time $\Omega(N)$, and that there exist non-partial order systems that can assemble shapes with diameter $N$ in time $o(N)$.
The model we use applies to both the seeded aTAM and the hierarchical aTAM.

\newcommand{\unrealisticHierarchical}{
    For hierarchical systems, our assembly time model may not be completely suitable since we make some potentially unrealistic assumptions.
    In particular, we ignore diffusion rates of molecules based on size and assume that large assemblies diffuse as fast as individual tiles.
    We also assume that the binding energy $\tau$ necessary for a small tile $t$ to attach stably to an assembly $\alpha$ is the same as the binding energy required for a large assembly $\beta$ to attach stably to $\alpha$, even though one would expect such large assemblies to have a higher reverse rate of detachment (slowing the net rate of forward growth) if bound with only strength $\tau$.
    However, from the perspective of our lower bound on assembly time, Theorem~\ref{thm-hier-partial-order-slow}, these assumptions have the effect of making hierarchial self-assembly appear \emph{faster}.
    We show that even with these extra assumptions, the time complexity of hierarchical partial order systems is \emph{still} no better than the seeded aTAM.
    However, caution is warranted in interpreting the upper bound result, Theorem~\ref{thm-fast-rectangle}, of a sublinear time assembly of a shape.
    As we discuss in Section~\ref{sec-conclusion}, a plausible treatment of diffusion rates -- together with our lower bound techniques based on low concentrations of large assemblies -- may yield an absolute linear-time (in terms of diameter) lower bound on assembly time of hierarchical systems, so that Theorem~\ref{thm-fast-rectangle} may owe its truth entirely to the heavily exploited assumption of equally fast diffusion of all assemblies.
    A reasonable interpretation of Theorem~\ref{thm-fast-rectangle} is that the partial order assumption is necessary to prove Theorem~\ref{thm-hier-partial-order-slow} and that concentration arguments alone do not suffice to establish linear-time time lower bounds in general hierarchical systems.
    The techniques that weave together both ``assembly parallelism'' and ``binding parallelism'', as discussed in Section~\ref{sec-intro} and Section~\ref{sec-fast-rectangle}, may prove useful in other contexts, even though their attained speedup is modest.
}

\opt{normal}{\unrealisticHierarchical}



\subsection{Definition of Time Complexity of Seeded Tile Systems}
\label{sec-seeded-time-defn}

We now review the definition of time complexity of seeded self-assembly proposed in~\cite{AdChGoHu01}.
A \emph{concentrations function} on a tile set $T$ is a subprobability measure $C:T \to [0,1]$ (i.e., $\sum_{r\in T} C(r) \leq 1$).
Each tile type $r$ is assumed to be held at a fixed concentration $C(r)$ throughout the process of assembly.\footnote{For singly-seeded tile systems in which the seed tile $s \in T$ appears only once at the origin, this assumption is valid in the limit of low seed concentration $C(s)$ compared to all other concentrations $C(r)$ for $r \in T \setminus \{s\}$.
\opt{normal}{This is because the number of terminal assemblies (if each is of size at most $K$) will be limited by $C(s)$, implying the percentage change in every other tile type $r$'s concentration is at most $K \cdot C(s) / C(r)$; therefore ``low'' seed concentration means setting $C(s) \ll C(r) / K$ for all $r \in T \setminus\{s\}$.
In fact, to obtain an assembly time asymptotically as fast, one need only ensure that for all $r$, $C(r) \geq 2 \#_{\ha}(r) C(s)$, where $\#_{\ha}(r)$ is the number of times $r$ appears in the terminal assembly $\ha$.
This guarantees that the concentration of $t$ is always at least half of its start value, which means that the assembly time, each step of which is proportional to the concentration of the tile type attaching at that step, is at most doubled compared to the case when the concentrations are held constant.}}
The assembly time for a seeded TAS $\calT=(T,\sigma,\tau)$ is defined by picking a copy of the seed arbitrarily and measuring the expected time before the seed grows into some terminal assembly, when assembly proceeds according to the following stochastic model.
The assembly process is described as a continuous-time Markov process in which each state represents a producible assembly, and the initial state is the seed assembly $\sigma$.
For each pair of producible assemblies $\alpha,\beta$ such that $\alpha \to_1 \beta$ via the addition of tile type $r$, there is a transition in the Markov process from state $\alpha$ to state $\beta$ with transition rate $C(r)$.\opt{normal}{\footnote{That is, the expected time until the next attachment of a tile to $\alpha$ is an exponential random variable with rate $\sum_{p\in\partial\alpha} C(\ha(p))$, where $\partial\alpha$ is frontier of $\alpha$, the set of empty locations at which a tile could stably attach to $\alpha$.
The probability that a particular $p'\in\partial\alpha$ leading to assembly $\beta$ is the next location of attachment is $C(\ha(p')) / \sum_{p\in\partial\alpha} C(\ha(p))$.}}
The sink states of the Markov process are precisely the terminal assemblies.
%If $\calT$ is directed, then $\ha$ is the unique sink state of the Markov process.
The time to reach some terminal assembly from $\sigma$ is a random variable $\time_{\calT,C}$, and the assembly time complexity of the seeded TAS $\calT$ with concentrations $C$ is defined to be $\mathsf{T}(\calT,C) = \exp{\time_{\calT,C}}$.
%Given a finite shape $S\subset \Z^2$, the \emph{(directed) seeded assembly time complexity} of $S$ is $\timeS(S) = \inf_{\calT,C} \mathsf{T}(\calT,C)$, where the infimum is over all directed seeded TAS's $\calT$ that strictly self-assembly $S$ and tile concentration functions $C$ to $\calT$.
%The authors of~\cite{AdChGoHu01} show that $\timeS(S_n) = \Theta(n)$, where $S_n$ is the $n \times n$ square.

The requirement that the tile concentrations function $C$ be a subprobability measure, rather than an arbitrary measure taking values possibly greater than 1, reflects a physical principle known as the \emph{finite density constraint}, which stipulates that a given unit volume of solution may contain only a bounded number of molecules (if for no other reason than to avoid forming a black hole).
By normalizing so that one ``unit'' of volume is the volume required to fit one tile, the total concentration of tiles (concentration defined as  number or mass per unit volume) cannot exceed 1.\opt{normal}{\footnote{When our goal is to obtain only an asymptotic result concerning a family of tile systems assembling a family of assemblies of size/diameter $N$, we may relax the finite density constraint to the requirement that the concentrations sum to a constant $c\in\R^+$ independent of $N$, since these concentrations could be divided by $c$ to sum to 1 while affecting the assembly time results by the same constant $c$, leaving the asymptotic results unaffected.}}
%By letting their total concentration be exactly 1, we are essentially requiring that the assembly process is carried out in the smallest volume (which leads to the fastest reaction time) required to satisfy the finite density constraint.
%This equality normalizes different systems for fair comparison of their respective time complexities.

We have the following time complexity lower bound for seeded systems.
This theorem says that even for non-directed systems, a seeded TAS can grow its diameter only linearly with time.
It strengthens and implies Lemma 4.6 of the full version of~\cite{AdChGoHu01}, which applied only to directed systems.
\opt{submission}{
    A proof of Theorem~\ref{thm-seeded-time-lower-bound} is contained in Section~\ref{app-sec-seeded-lower-bound}.
}

\newcommand{\seededLowerBoundFormal}{
    Let $d \in \Z^+$.
    Let $\calT=(T,\sigma,\tau)$ be a singly-seeded TAS (meaning $|\sigma|=1$), and let $C:T\to[0,1]$ be a concentrations function.
    Since it takes only constant time for the assembly to grow to any constant radius, restricting attention to singly-seeded systems does not asymptotically affect the result for tile systems with a finite seed assembly of size larger than 1.
    %We say that $\calT$ is \emph{$d$-wide} if, for all $\ha \in \termasm{\calT}$, some point in $\dom \ha$ is at least distance $d$ (in the $L_1$ norm) from the seed.
    %In other words, we require that $\calT$ is guaranteed to grow to at least distance $d$ from the seed.\footnote{Otherwise it does not make sense to ask how long it takes to grow to distance $d$.  Alternately, we could have formulated the statement as the expected time to grow to distance $d$, conditioned on the event that growth ever reaches distance $d$, but }
    Let $\mathbf{D}(\calT,C,d)$ be the random variable representing the time that any tile is first placed at distance $d$ (in the $L_1$ norm) from the seed, conditioned on the event that a tile is eventually placed at least distance $d$ from the seed, with $\mathbf{D}(\calT,C,d)=\infty$ if all producible, terminal assemblies of $\calT$ are completely contained in radius $d-1$ around the seed.
}

\opt{normal}{\seededLowerBoundFormal}

\newcommand{\seededLowerBoundFormalStatement}{For each $d \in \Z^+$, each singly-seeded TAS $\calT$, and each concentrations function $C:T\to[0,1]$, $\exp{\mathbf{D}(\calT,C,d)} = \Omega(d)$.}

\newcommand{\seededLowerBoundInformalStatement}{For any seeded TAS $\calT$ and any concentrations function on $\calT$, the expected time at which the assembly formed by $\calT$ grows to diameter $d$ is $\Omega(d)$.}

\begin{theorem}\label{thm-seeded-time-lower-bound}
\opt{normal}{\seededLowerBoundFormalStatement}
\opt{submission}{\seededLowerBoundInformalStatement}
\end{theorem}

\newcommand{\ProofSeededTimeLowerBound}{
    Since we care only about the first time at which a tile is attached at distance $d$ (before which there are no tiles at distance $d'$ for any $d' \geq d$), we can restrict the assembly process to the region of radius $d$ around the seed.
    Therefore we model the assembly process as if it proceeds normally until the first tile attaches at distance $d$ from the seed, at which point all growth immediately halts.
    %We state the proof only for \emph{singly-seeded} tile systems, meaning those with a single seed tile.

    Define $\R^+ = [0,\infty)$.
    Given $i \in \{0,\ldots,d\}$ and $t \in \R^+$, let $\mathbf{X}_i(t)$ be a random variable denoting the number of tiles attached at locations with distance exactly $i$ from the seed at time $t$, under the restriction stated above that all assembly halts the moment that a tile is placed at distance $d$.
    Then for all $t\in\R^+$, the event $\mathbf{X}_d(t) = 0$ (no tile is at distance $d$ by the time $t$) is equivalent to the event $\mathbf{D}(\calT,C,d) > t$ (the time of the first attachment at distance $d$ strictly exceeds $t$).
    %Once this time has passed, the variables $X_i(t)$ no longer model the assembly process accurately, but since we

    %Note that if $\calT$ cannot grow to distance $i > d$, then $\mathbf{X}_i(t) = 0$ for all $t\in\R^+$.
    In a seeded TAS, tiles can attach at a location only when there is another tile adjacent to the location.
    Locations at $L_1$-distance $i$ to the seed are only adjacent to locations at distance either $i+1$ or $i-1$ to the seed.
    Off the $x$- and $y$-axes, each location at distance $i$ has two neighbors at distance $i-1$ and two neighbors at distance $i+1$, and for the 4 locations at distance $i$ on either axis, every location has one neighbor at distance $i-1$ and three neighbors at distance $i+1$.
    Therefore, at time $t$, tiles are attachable to at most $3 \mathbf{X}_{i-1}(t) + 2 \mathbf{X}_{i+1}(t)$ different locations with distance $i$ to the seed.
    %Let $\alpha$ be an assembly, let $p \in \partial \alpha$, and let $\{\beta_1,\ldots,\beta_k\}$ denote the set of assemblies such that $\alpha \to_1 \beta_i$ via attachment at location $p$.
    %Since $\sum_{r \in T} C(r) = 1$, this implies that the rate of attachment to $\alpha$ at location $p$ is $\sum_{}$.
    Since the total concentration of any single tile type is at most $1$, the rate at which tiles attach at any given location is at most $1$.
    For all $i\in\{0,\ldots,d\}$, define the function $f_i:\R^+ \to \R^+$ for all $t\in\R^+$ by $f_i(t) = \exp{\mathbf{X}_i(t)}$.
    Then for $i\in\{1,\ldots,d-1\}$,
    \[
    \frac{df_i(t)}{dt}\ \leq\ 3f_{i-1}(t)\ +\ 2f_{i+1}(t),
    %\]
    \text{ and }
    %\[
    \frac{df_d(t)}{dt}\ \leq\ 3f_{d-1}(t).
    \]
    The lack of a $2f_{d+1}(t)$ term in the latter inequality is due to our modification of the assembly process to immediately halt once the first tile attaches at distance $d$.
    Since the assembly process always starts with a single seed tile, $f_0(t)=1$ for all $t\in\R^+$, and $f_i(0) = 0$ for all $i \in \{0,\ldots,d\}$.
    For all $t\in\R^+$ and all $i\in\{1,\ldots,d\}$, $f_i(t) \leq 4i$ since there are exactly $4i$ locations at distance exactly $i$ to the seed.
    %To prove the theorem, we only need to focus on when the first tile attaches at distance $d$. Until that time, no tile will be able to attach at distance larger than $d$.

    Let $t_0 \in \R^+$ be the unique time at which $f_d(t_0) = \frac{1}{2}.$
    This time is unique since $f_d$ is monotonically increasing.
    Since $f_d(t_0) = \exp{\mathbf{X}_d(t_0)}$, by Markov's inequality, $\prob[\mathbf{X}_d(t_0) \geq 1] \leq \frac{1}{2}$, implying that $\prob[\mathbf{X}_d(t_0) < 1] > \frac{1}{2}$.
    Since $\mathbf{X}_d$ is integer-valued and nonnegative, this is equivalent to stating that $\prob[\mathbf{X}_d(t_0) = 0] > \frac{1}{2}$.
    Recall that $\mathbf{X}_d(t_0) = 0 \iff \mathbf{D}(\calT,C,d) > t_0$,  whence $\prob[\mathbf{D}(\calT,C,d) > t_0] > \frac{1}{2}$.
    By Markov's inequality, $\exp{\mathbf{D}(\calT,C,d)} > \frac{t_0}{2}$.
    Thus it suffices to prove that $t_0 \geq \Omega(d)$.
    To do this, we define a simpler function that is an upper bound for $f_d$ and solve its differential equations.

    %Since this means that if we do not allow tiles to attach at distance $d+1$ or more, then at least half of the instances, no tiles attach at distance $d$ within time $\frac{d}{c}$ and thus the average time for any tile to attach at distance $d$ to the seed is at least $\frac{d}{2c}$. In the rest of the proof, we focus on giving an upper bound on $f_d(t)$ subject to $f_{i}(t) = 0$ for all $t$ and all $i >d$.

    For all $i\in\{0,\ldots,d\}$, define the function $g_i:\R^+ \to \R^+$ (which will serve as an upper bound for $f_i$) as follows.
    For all $1\in\{1,\ldots,d-1\}$,
    \[
    \frac{dg_i(t)}{dt}\ =\ 3g_{i-1}(t)\ +\ 2g_{i+1}(t),\ \mbox{when $g_i(t) < 4d$},
    \]
    \[
    \frac{dg_d(t)}{dt}\ =\ 3g_{d-1}(t),\ \mbox{when $g_d(t) < 4d$},
    \]
    and for all $i\in\{0,\ldots,d\}$,
    \[
    \frac{dg_i(t)}{dt}\ =\ 0,\ \mbox{when $g_i(t) = 4d$},
    \]
    with the boundary conditions $g_0(t)=4d$ for all $t \in \R^+$, $g_i(0) = 0$ for all $i \in \{1,\ldots,d\}$.
    It is routine to check that $g_i(t) \geq f_i(t)$ for all $i\in\{0,\ldots,d\}$ and $t\in\R^+$. Furthermore, if $g_i(t_0) > g_{i+1}(t_0)$ for all $i\in\{0,\ldots,d\}$ and a specific time point $t_0 \in \R^+$, then
    \[
    \frac{dg_i(t)}{dt}\ \geq\ \frac{dg_{i+1}(t)}{dt}\ \mbox{at time $t_0$},
    \]
    Since $g_i(0) \geq g_{i+1}(0)$ for all $i\in\{0,\ldots,d\}$ by definition, we know that $g_i(t) \geq g_{i+1}(t)$ for all $i\in\{0,\ldots,d\}$ and all $t\in\R^+$.
    Using this monotonicity, we can define a set of functions $h_i(t)$ that are upper bounds for $g_i(t)$ by the following.
    \[
    \frac{dh_i(t)}{dt}\ =\ 5h_{i-1}(t) \mbox{, for all $i\in\{1,\ldots,d\}$}, \text{ and } \frac{dh_0(t)}{dt} = 0,
    \]
    with boundary conditions $h_0(t)=4d$ for all $t\in\R^+$, $h_i(0) = 0$ for all $i\in\{0,\ldots,d\}$. Solving these differential equations, we obtain $h_d(t)=\frac{4d}{d!}(5t)^d$.  Letting $t'=\frac{d}{10e}$, by Stirling's inequality $d! > \sqrt{2 \pi d} \left( \frac{d}{e} \right)^d e^{1 / (12 d + 1)} > \left( \frac{d}{e} \right)^d$, we have
    \[
    f_d\left(t'\right)
    \leq
    g_d\left(t'\right)
    \leq
    h_d\left(t'\right)
    =
    \frac{4d}{d!} \cdot \left(5t'\right)^d
    =
    \frac{4d}{d!} \cdot \left( \frac{d}{2 e} \right)^d
    <
    \frac{4d}{\left( \frac{d}{e} \right)^d} \cdot \left( \frac{d}{2 e} \right)^d
    =
    \frac{4d}{2^d}.
    \]
    %The last inequality follows from Stirling's inequality $d! > \sqrt{2 \pi d} \left( \frac{d}{e} \right)^d e^{1 / (12 d + 1)}$.
    Since $f_d$ is monotonically increasing, $f_d(t_0) = \frac{1}{2}$ by definition, and $\frac{4d}{2^d} < \frac{1}{2}$ for sufficiently large $d$, this implies that $t_0 > t' = \frac{d}{10e}$.
}

\opt{normal}{
    \begin{proof}
      \ProofSeededTimeLowerBound
    \end{proof}
}



















\subsection{Definition of Time Complexity of Hierarchical Tile Systems}
\label{sec-time-complexity-hierarchical}


To define time complexity for hierarchical systems, we employ more explicitly the chemical kinetics that implicitly underlie the time complexity model for seeded systems stated in Section~\ref{sec-seeded-time-defn}.
We treat each assembly as a single molecule. If two assemblies $\ta$ and $\tb$ can attach to create an assembly $\tg$, then we model this as a chemical reaction $\ta + \tb \to \tg$, in which the rate constant is assumed to be equal for all reactions (and normalized to 1).
In particular, if $\ta$ and $\tb$ can be attached in two different ways, this is modeled as two different reactions, even if both result in the same assembly.\opt{normal}{\footnote{The fact that some directed systems may not require at least one of these attachments to happen in every terminal assembly tree is the reason we impose the partial order requirement when proving our time complexity lower bound.}}


At an intuitive level, the model we define can be explained as follows.
We imagine dumping all tiles into solution at once, and at the same time, we grab one particular tile and dip it into the solution as well, pulling it out of the solution when it has assembled into a terminal assembly.
Under the seeded model, the tile we grab will be a seed, assumed to be the only copy in solution (thus requiring that it appear only once in any terminal assembly).
In the seeded model, no reactions occur other than the attachment of individual tiles to the assembly we are holding.
In the hierarchical model, other reactions are allowed to occur in the background (we model this using the standard mass-action model of chemical kinetics~\cite{epstein1998introduction}), but only those reactions with the assembly we are holding move us ``closer'' to completion.
The other background reactions merely change concentrations of other assemblies (although these indirectly affect the time it will take our chosen assembly to complete, by changing the rate of reactions with our chosen assembly).


One reason for choosing this model is that we would like to analyze the assembly time in such as way as to facilitate direct comparison with the results of~\cite{AdChGoHu01}.
In particular, we would like the assembly time model proposed in~\cite{AdChGoHu01} to be derived as a special case of the model we propose, when only single-tile reactions with the seed-containing assembly are allowed.
With a model such as Gillespie's algorithm~\cite{Gillespie77,GibsonBruck00,Gillespie07} using finite molecular counts, it is possible that no copy of the terminal assembly forms, so it is not clear how to sensibly ask how long it takes to form.\footnote{This problem is easily averted in a seeded system by setting the seed concentration sufficiently low (but still $\Omega(|T|)$) to ensure that the terminal assembly is guaranteed to form at least one copy.  In a hierarchical system it is not clear how to avoid this problem.}
The mass-action model of kinetics~\cite{epstein1998introduction} describes concentrations as a dynamical system that evolves continuously over time according to ordinary differential equations derived from reaction rates.
This is an accepted model of kinetics when molecular counts are very large, which is already an implicit assumption in the standard aTAM.
In the mass-action model, all possible terminal assemblies (assuming there are a finite number of different terminal assemblies) are guaranteed to form, which resolves one issue with the purely stochastic model.
But the solution goes too far: some (infinitesimal) concentration of all terminal assemblies form in the first infinitesimal amount of time.
A sensible way to handle this may be to measure the time to half-completion (time required for the concentration of a terminal assembly to exceed half of its steady-state concentration.
But this model is potentially subject to ``cheats'' such as systems that ``kill'' all but the fastest growing assemblies, so as to artificially inflate the average time to completion of those that successfully assemble into the terminal assembly.
Furthermore, it would not necessarily be fair to directly compare such a deterministic model with the stochastic model of~\cite{AdChGoHu01}.
%This is like moving the finish line closer so that it takes less time to get halfway to it.

The model of assembly time that we define is a continuous-time stochastic model similar to that of~\cite{AdChGoHu01}.
However, rather than fixing transition rates at each time $t\in\R^+$ as constant, we use mass-action kinetics to describe the evolution over time of the concentration of producible assemblies, including individual tile types, which in turn determine transition rates.
To measure the time to complete a terminal assembly, we use the same stochastic model as~\cite{AdChGoHu01}, which fixes attention on one particular tile and asks what is the expected time for it to grow into a terminal assembly, where the rate of attachment events that grow it are time-dependent, governed by the continuous mass-action evolution of concentration of assemblies that could attach to it.
Unlike the seeded model, we allow the tile concentrations to deplete, since it is no longer realistic (or desirable for nontrivial hierarchical constructions) to assume that individual tiles do not react until they encounter an assembly containing the seed.\footnote{However, this depletion of individual tiles is \emph{not} the source of our time lower bound.  Suppose that we used a transition rate of 1 for each attachment of an individual tile (which is an upper bound on the attachment rate even for seeded systems due to the finite density constraint) and dynamic transition rates only for attachment of larger assemblies.  Then the assembly of hierarchical partial order systems \emph{still} would proceed asymptotically no faster than if single tile attachments were the only reactions allowed (as in the seeded assembly case), despite the fact that all the single-tile reactions at the intersection of the seeded and hierarchical model would be at least as fast in the modified hierarchical model as in the seeded model.}






We first formally define the dynamic evolution of concentrations by mass-action kinetics.
Let $\calT=(T,\tau)$ be a hierarchical TAS, and let $C:T\to[0,1]$ be a concentrations function.
Let $\R^+ = [0,\infty)$, and let $t\in\R^+.$
For $\alpha\in\prodasm{\calT}$, let $[\alpha]_C(t)$ (abbreviated $[\alpha](t)$ when $C$ is clear from context) denote the concentration of $\alpha$ at time $t$ with respect to initial concentrations $C$, defined as follows.\opt{normal}{\footnote{More precisely, $[\alpha](t)$ denotes the concentration of the equivalence class of assemblies that are equivalent to $\alpha$ up to translation.  We have defined assemblies to have a fixed position only for mathematical convenience in some contexts, but for defining concentration, it makes no sense to allow the concentration of an assembly to be different from one of its translations.}}
We often omit explicit mention of $C$ and use the notation $[r](0)$ to mean $C(r)$, for $r\in T$, to emphasize that the concentration of $r$ is not constant with respect to time.
Given two assemblies $\alpha$ and $\beta$ that can attach to form $\gamma$, we model this event as a chemical reaction $R: \alpha + \beta \to \gamma$.
Say that a reaction $\alpha+\beta\to\gamma$ is \emph{symmetric} if $\alpha=\beta$.
Define the \emph{propensity} (a.k.a., \emph{reaction rate}) of $R$ at time $t\in\R^+$ to be $\rho_R(t) = [\alpha](t) \cdot [\beta](t)$ if $R$ is not symmetric, and $\rho_R(t) = \frac{1}{2} \cdot [\alpha](t)^2$ if $R$ is symmetric.\opt{normal}{\footnote{That is, all reaction rate constants are equal to 1.  To the extent that a rate constant models the ``reactivity'' of two molecules (the probability that a collision between them results in a reaction), it seems reasonable to model the rate constants as being equal.
To the extend that a rate constant also models diffusion rates, this assumption may not apply; we discuss the issue in Section~\ref{sec-conclusion}.
Since we are concerned mainly with asymptotic results, if rate constants are assumed equal, it is no harm to normalize them to be 1.}}

If $\alpha$ is consumed in reactions $\alpha + \beta_1 \to \gamma_1, \ldots, \alpha + \beta_n \to \gamma_n$ and produced in asymmetric reactions $\beta'_1 + \gamma'_1 \to \alpha, \ldots, \beta'_m + \gamma'_m \to \alpha$ and symmetric reactions $\beta''_1 + \beta''_1 \to \alpha, \ldots, \beta''_p + \beta''_p \to \alpha$, then the concentration $[\alpha](t)$ of $\alpha$ at time $t$ is described by the differential equation
\begin{equation}\label{eq-conc-diff}
    \frac{d [\alpha](t)}{d t} =
    \sum_{i=1}^m [\beta'_i](t) \cdot [\gamma'_i](t)
    + \sum_{i=1}^p \frac{1}{2} \cdot  [\beta''_i](t)^2
    - \sum_{i=1}^n [\alpha](t) \cdot [\beta_i](t),
\end{equation}
with boundary conditions $[\alpha](0) = C(r)$ if $\alpha$ is an assembly consisting of a single tile $r$, and $[\alpha](0) = 0$ otherwise.
In other words, the propensities of the various reactions involving $\alpha$ determine its rate of change, negatively if $\alpha$ is consumed, and positively if $\alpha$ is produced.
\opt{submission}{The above definitions of propensities are intuitively justified in Section \ref{sec-propensity-explanation}.}

\newcommand{\propensityExplanation}{
    The definitions of the propensities of reactions deserve an explanation.
    Each propensity is proportional to the average number of collisions between copies of reactants per unit volume per unit time.
    For a symmetric reaction $\beta'' + \beta'' \to \alpha$, this collision rate is half that of the collision rate compared to the case where the second reactant is a distinct type of assembly, assuming it has the same concentration as the first reactant.\footnote{For intuition, consider finite counts: with $n$ copies of $\gamma$ and $n$ copies of $\beta \neq \gamma$, there are $n^2$ distinct pairs of molecules of respective type $\gamma$ and $\beta$, but with only $n$ copies of $\gamma$, there are $\frac{n(n-1)}{2}$ distinct pairs of molecules of type $\gamma$, which approaches $\frac{1}{2}n^2$ as $n \to \infty$.}
    Therefore the amount of $\alpha$ produced per unit volume per unit time is half that of a corresponding asymmetric reaction.
    The reason that terms of symmetric reactions $\alpha+\alpha\to\gamma$ that \emph{consume} $\alpha$ are not corrected by factor $\frac{1}{2}$ is that, although the number of such reactions per unit volume per unit time is half that of a corresponding asymmetric reaction, each such reaction consumes two copies of $\alpha$ instead of one.
    This constant 2 cancels out the factor $\frac{1}{2}$ that would be added to correct for the symmetry of the reaction.
    Therefore, the term $[\alpha](t) \cdot [\beta_i](t)$ representing the rate of consumption of $\alpha$ is the proper value whether or not $\alpha=\beta_i$.
}
\opt{normal}{\propensityExplanation}

%\opt{normal}{
%    Of course, many hierarchical tile assembly systems will have the property that no producible assembly is attachable to itself.
%    In this case, equation \eqref{eq-conc-diff} reduces to
%    \begin{equation}\label{eq-conc-diff-unique-reactants}
%        \frac{d [\alpha](t)}{d t} =
%        \sum_{i=1}^m [\beta'_i](t) \cdot  [\gamma'_i](t)
%        - \sum_{i=1}^n [\alpha](t) \cdot  [\beta_i](t),
%    \end{equation}
%}

This completes the definition of the dynamic evolution of concentrations of producible assemblies; it remains to define the time complexity of assembling a terminal assembly.
%Suppose $\calT$ is directed.
%Then let $\ha\in\termasm{\calT}$ be its unique producible, terminal assembly.
Although we have distinguished between seeded and hierarchical systems, for the purpose of defining a model of time complexity in hierarchical systems and comparing them to the seeded system time complexity model of~\cite{AdChGoHu01}, it is convenient to introduce a seed-like ``timekeeper tile'' into the hierarchical system, in order to stochastically analyze the growth of this tile when it reacts in a solution that is itself evolving according to the continuous model described above.
The seed does not have the purpose of nucleating growth, but is introduced merely to focus attention on a single molecule that has not yet assembled anything, in order to ask how long it will take to assemble into a terminal assembly.\footnote{For our lower bound result, Theorem~\ref{thm-hier-partial-order-slow}, it will not matter which tile type is selected as the timekeeper, except in the following sense.  We define partial order systems, the class of directed hierarchical TAS's to which the bound applies, also with respect to a particular tile type in the unique terminal assembly.  A TAS may be a partial order system with respect to one tile type but not another, but for all tile types $s$ for which the TAS is a partial order system, the time lower bound of Theorem~\ref{thm-hier-partial-order-slow} applies when $s$ is selected as the timekeeper.
The upper bound of Theorem~\ref{thm-fast-rectangle} holds with respect to only a single tile type, which will appear at a unique position in the final assembly.}
The choice of which tile type to pick will be a parameter of the definition, so that a system may have different assembly times depending on the choice of timekeeper tile.

%Let $\ha$ be the unique terminal assembly of the hierarchical TAS.
%Each producible, terminal assembly $\ha\in\termasm{\calT}$ will be the sink state of a Markov process.
Fix a copy of a tile type $s$ to designate as a ``timekeeper seed''.
The assembly of $s$ into some terminal assembly $\ha$ is described as a time-dependent continuous-time Markov process in which each state represents a producible assembly containing $s$, and the initial state is the size-1 assembly with only $s$.
For each state $\alpha$ representing a producible assembly with $s$ at the origin, and for each pair of producible assemblies $\beta,\gamma$ such that $\alpha + \beta \to \gamma$ (with the translation assumed to happen only to $\beta$ so that $\alpha$ stays ``fixed'' in position), there is a transition in the Markov process from state $\alpha$ to state $\gamma$ with transition rate $[\beta](t)$.\footnote{That is, for the purpose of determining the continuous dynamic evolution of the concentration of assemblies, including $\alpha$,  in solution at time $t$, the rate of the reaction $\alpha + \beta \to \gamma$ at time $t$ is assumed to be proportional to $[\alpha](t)[\beta](t)$ (or half this value if the reaction is symmetric).
However, for the purpose of determining the stochastic dynamic evolution of one particular copy of $s$, the rate of this reaction at time $t$ is assumed to be proportional only to $[\beta](t)$.
This is because we want to describe the rate at which \emph{this particular copy} of $\alpha$, the one containing the copy of $s$ that we fixed at time 0, encounters assemblies of type $\beta$.
This instantaneous rate is independent of the number of \emph{other} copies of $\alpha$ at time $t$ (although after $\epsilon$ seconds the rate will change to $[\beta](t+\epsilon)$, which of course \emph{will} depend on $[\alpha]$ over that time interval).}
Unlike the seeded model, the transition rates vary over time since the assemblies (including assemblies that are individual tiles) with which $s$ could interact are themselves being produced and consumed.


We define $\time_{\calT,C,s}$ to be the random variable representing the time taken for the copy of $s$ to assemble into a terminal assembly via some sequence of reactions as defined above.
%Note in particular that unlike the seeded model, there are other reactions occurring outside the sequence, between two assemblies $\alpha$ and $\beta$ that do not contain the timekeeper tile.
%However, these (continuously and deterministically modeled) reactions will determine the concentration of tiles and assemblies that in turn determine the propensities of (discretely and stochastically modeled) reactions that \emph{do} involve the timekeeper.
We define the time complexity of a directed hierarchical TAS $\calT$ with concentrations $C$ and timekeeper $s$ to be $\mathsf{T}(\calT,C,s) = \exp{\time_{\calT,C,s}}$.
It is worth noting that this expected value could be infinite.
This would happen if some partial assembly $\alpha$, in order to complete into a terminal assembly, requires the attachment of some assembly $\beta$ whose concentration is depleting quickly.
%Given a finite shape $S\subset \Z^2$, the \emph{(directed) hierarchical assembly time complexity} of $S$ is $\timeH(S) = \inf_{\calT,C} \max_{p\in\dom\ha(\calT)} \mathsf{T}(\calT,C,p)$, where the infimum is over all directed hierarchical TAS's $\calT$ that strictly self-assembly $S$, tile concentration functions $C$ to $\calT$, and $\ha(\calT)$ is defined to be the unique terminal assembly of $\calT$.


We note in particular that our construction of Theorem~\ref{thm-hierarchical-square} is composed of $(\frac{n}{\log n})^2$ different types of $O(\log n) \times O(\log n)$ ``blocks'' that can each grow via only one reaction.
At least one of these blocks $\beta$ must obey $[\beta](t) \leq \frac{\log^2 n}{n^2}$ for all $t\in\R^+$.
This implies that the rate of the slowest such reaction is at most $\frac{\log^2 n}{n^2}.$
Thus our square construction assembles in at least $\Omega(\frac{n^2}{\log^2 n})$ time, slower than the optimal seeded time of $O(n)$ \cite{AdChGoHu01}.
Proving this formally requires more details that we omit, but the fact that the system is a partial order system as defined in Section~\ref{sec-defn-partial-order-systems} means that Theorem~\ref{thm-hier-partial-order-slow} implies a time complexity lower bound of $\Omega(n)$.
























==> two-handed-square.tex <==

\section{Nearly Maximally Parallel Hierarchical Assembly of an $n \times n$ Square with Optimal Tile Complexity}
\label{sec-hierarchical-square}

In this section we show that under the hierarchical model of tile assembly, it is possible to self-assemble an $n \times n$ square, for arbitrary $n \in \Z^+$, using the asymptotically optimal $O(\frac{\log n}{\log \log n})$ number of tile types.
Furthermore, the square assembles using nearly the maximum possible parallelism in the hierarchical model, building the final square out of four assembled sub-squares of size $n/2 \times n/2$, which are themselves each assembled from four sub-squares of size $n/4 \times n/4$, etc.
\opt{normal}{
The sub-optimality stems from the need for us to construct the smallest sub-squares of size $O(\log n) \times O(\log n) = O(\log^2 n)$ without parallelism.
}

\opt{normal}{
    We formalize the notion of ``parallelism through hierarchical assembly'' as follows.
}


\newcommand{\FigSquareHighLevelCaption}{
  Overview of the hierarchical TAS that assembles an $n \times n$ square with $O(\log^2 n)$ assembly depth and $O(\frac{\log n}{\log \log n})$ tile complexity.
  Each square in the figure represents a block of width $O(\log n)$ with each side of each block encoding its $(x,y)$-address in the square.
  \opt{normal}{(The encoding scheme is shown in more detail in Figure~\ref{fig:two-handed-square-block}.)}
  Each of the thin solid lines is a strength-1 glue; in fact they are all identical.
  Dotted lines connect those glues that are intended to bind to each other.
  The circled subassemblies show the order of growth of one particular block (at coordinates $(3,2)$) into the final square.
}

\opt{submission}{
    \newcommand{\twoHandedSquareFigWidth}{3.5in}
    \begin{wrapfigure}{r}{\twoHandedSquareFigWidth}
    \vspace{-15pt}
      \begin{center}
      \includegraphics[width=\twoHandedSquareFigWidth]{figures/two-handed-square-high-level}
      \caption{\label{fig:two-handed-square-high-level} \figuresize
      \FigSquareHighLevelCaption}
      \end{center}
    \vspace{-30pt}
    \end{wrapfigure}
}



\opt{submission}{
We give a formal definition of ``parallelism through hierarchical assembly'' in Section~\ref{sec-app-parallel-square}, which defines $\Kddac(\calT)$ as the maximum depth of any ``assembly tree'' of $\calT$.
}

\newcommand{\ParallelDefn}{
    Let $\calT=(T,\tau)$ be a directed hierarchical TAS.
    Let $\alpha \in \prodasm{\calT}$ be a producible assembly.
    An \emph{assembly tree} $\Upsilon$ of $\alpha$ is a binary tree whose nodes are labeled by producible assemblies, with $\alpha$ labeling the root, individual tile types labeling the $| \alpha|$ leaves, and node $v$ having children $u_1$ and $u_2$ with the requirement that $u_1$ and $u_2$ can attach to assemble $v$.
    That is, $\Upsilon$ represents one possible pathway through which $\alpha$ could be produced from individual tile types in $\calT$.
    Let $\Upsilon(\calT)$ denote the set of all assembly trees of $\calT$.
    Say that an assembly tree is \emph{terminal} if its root is a terminal assembly.
    %An assembly can be terminal even if T is not directed, so we can define a terminal assembly tree for any TAS, not just terminal systems.
    Let $\Upsilon_\Box(\calT)$ denote the set of all terminal assembly trees of $\calT$.
    Note that even a directed hierarchical TAS can have multiple terminal assembly trees that all have the same root terminal assembly.
    The \emph{assembly depth} of $\calT$ is
    $
        \Kddac(\calT) = \max_{\Upsilon \in \Upsilon_\Box(\calT)} \mathrm{depth}(\Upsilon),
    $
    where $\mathrm{depth}(\Upsilon)$ denotes the standard depth of the tree $\Upsilon$, the length of the longest path from any leaf to the root.

    %Let $S \subset \Z^2$ be a finite shape.
%    The \emph{directed assembly depth} of $S$ is
%    $$\Kddac(S) = \min \setr{\Kddac(\calT)}{\begin{array}{l}
%    \calT=(T,\tau) \text{ is a directed hierarchical}
%    \\
%    \text{TAS and } \calT \text{ strictly self-assembles } S
%    \end{array}}.$$


     It is clear by the definition that for any shape $S$ with $N$ points strictly self-assembled by a tile system $\calT$, $\Kddac(\calT) \geq \log N$.
     Our construction nearly achieves this bound in the case of assembling an $n \times n$ square $S_n$, while simultaneously obtaining optimal tile complexity $O(\frac{\log n}{\log \log n})$.
     In other words, not only is it the case that every producible assembly can assemble into the terminal assembly (by the definition of directed), but in fact every producible assembly is at most $O(\log^2 n)$ attachment events from becoming the terminal assembly.

     %Furthermore, we achieve nearly optimal tile complexity in additional to optimal assembly depth.
     In~\cite{AGKS05}, the authors prove that whenever $n \in \N$ is algorithmically random, at least $\Omega(\log n / \log \log n)$ tile types are required to strictly self-assemble an $n \times n$ square in the hierarchical model.
     Actually, that paper states only that this holds for the \emph{$q$-tile model}, in which some constant $q$ exists that limits the size of attachable assemblies other than those containing a special seed tile, and the authors claim that the proof requires the bound $q$, but in fact their proof does not use the bound $q$ and works for the general hierarchical model~\cite{RobbiePersonal2010}.
}

\opt{normal}{\ParallelDefn}









\opt{normal}{
    \begin{figure}[htb]
    \begin{center}
      \includegraphics[width=5.7in]{figures/two-handed-square-high-level}
      \caption{\label{fig:two-handed-square-high-level} \figuresize
      \FigSquareHighLevelCaption
      }
    \end{center}
    \end{figure}
}



\newcommand{\FigNonPowTwo}{
    \begin{figure}[htb]
    \begin{center}
      \includegraphics[width=4in]{figures/two-handed-square-non-power-of-2}
      \caption{\label{fig:two-handed-square-non-power-of-2} \figuresize
      Design of block sizes to handle values of $n$ that are not a power of two. There are always exactly $2^k \times 2^k$ blocks, where $2^k \leq n < 2^{k+1}$.
      Each block doubles the length of its along the $x$-axis (resp. $y$-axis) if $n - 2^k$ exceeds its $x$-coordinate (resp. $y$-coordinate).
      %The solid lines represent block boundaries, and the dotted lines are to help visualize the size of the square.
      }
    \end{center}
    \end{figure}
}


\newcommand{\FigBlock}{
    \begin{figure}[htb]
    \begin{center}
      \includegraphics[width=6.5in]{figures/two-handed-square-block}
      \caption{\label{fig:two-handed-square-block} \figuresize
      Assembly of $O(\log n) \times O(\log n)$ size block from $O(\frac{\log n}{\log \log n})$ tile types.
      Every block starts from the same tile types that encode $n-2^k$, using exactly $k$ bits; in this example, $n=22$ so $k=4$ and $n-2^k$ is 0110 in binary using 4 bits.
      Thick solid lines represent strength-2 glues.
      For clarity, strength-1 glues are shown selectively to help verify that a certain order of growth is possible to enforce.
      The tiles encode $n-2^k$ in base $b$ chosen to be a power of two such that $\frac{\log n}{\log \log n} \leq b < 2  \frac{\log n}{\log \log n}$ (labeled ``seed'' for intuition, although those tiles start unattached).
      A constant-size set of tile types does the rest.
      $n-2^k$ is first converted to binary and each of its bits quadrupled to make room for the bumps and dents.
      Then $x$ and $y$ coordinates are randomly guessed and simultaneously compared to $n-2^k$; if either is smaller, that dimension is doubled in length (in this example the height is doubled but not the width).
      At the same time, the values of $x$ and $y$ are compared as described in the proof of Theorem~\ref{thm-hierarchical-square} to determine where to place strength-1 glues.}
    \end{center}
    \end{figure}
}

\opt{normal}{
    \FigNonPowTwo

    \FigBlock
}


\begin{theorem} \label{thm-hierarchical-square}
    For all $n\in\N$, there is a hierarchical TAS $\calT=(T,2)$ such that $\calT$ strictly self-assembles an $n \times n$ square, $|T| = O(\frac{\log n}{\log \log n})$, and $\Kddac(\calT) = O(\log^2 n)$.
   %There are constants $c_1,c_2\in\N$ such that, for all $n\in\N$, there is a directed hierarchical TAS $\calT=(T,2)$ such that $\calT$ strictly self-assembles the $n \times n$ square, $|T| \leq c_1 \log n / \log \log n$, and $\Kddac(\calT) \leq c_2 \log^2 n$.
\end{theorem}

\opt{submission}{
    A formal proof of Theorem~\ref{thm-hierarchical-square} is contained in Section~\ref{sec-app-parallel-square}.
    Figure~\ref{fig:two-handed-square-high-level} shows the high-level idea.
    The figure shows how to create a square of $n \times n$ blocks, each of width $O(\log n)$, for $n$ a power of two.
    The full proof explains how to handle $n$ that are not a power of two and how to handle $n$ that are not perfectly divisible by the block length.
    Intuitively, tiles aggregate into blocks while randomly guessing their ``$(x,y)$ address'' in the final square.
    The blocks encode this address into the bumps and dents on the side of the block, which ensures that fully formed blocks can only bind to their neighbors (the strength-1 glues shown in Figure~\ref{fig:two-handed-square-high-level} are all identical so the bumps and dents are required to encode this specificity.)
    The growth order of the blocks enforces that the strength-1 glues needed for binding are not present until enough bumps and dents are present to enforce this binding specificity.
    The $(x,y)$ address is also used to determine where to put strength-1 glues, since not all sides of all blocks have them.
    This enforces the ``recursive doubling'' of Figure~\ref{fig:two-handed-square-high-level}, namely that all blocks bind without overlap, so that blocks at level $i$ of the recursive hierarchy cannot bind to their level $i$ ``twin'' set of blocks until both have completely finished all level $i-1$ binding.
}


\newcommand{\ProofParallelSquare}{
   A high-level outline of the construction is shown in Figure~\ref{fig:two-handed-square-high-level}.
   We assemble a number of blocks of width $O(\log n) \times O(\log n)$, each of which represents in its tile types an address indicating its position in the square, and the block binds only to (some of) its neighboring blocks.
   The blocks assemble using standard single-tile accretion (actually we cannot directly enforce this in the model, but each block will nonetheless assemble the same structure in either model).
   Since each block is $O(\log^2 n)$ total tiles, this is the source of the suboptimal $O(\log^2 n)$ assembly depth.
   Once the blocks are assembled, however, they assemble into the full square using $O(\log n)$ assembly depth.
   All blocks $(x,y)$ with $x$ even bind to $(x+1)$ to create the two-block assembly $(x,y):(x+1,y)$, then all blocks $(x,y):(x+1,y)$ with $y$ even bind to $(x,y+1):(x+1,y+1)$ to create the four-block assembly $(x,y):(x+1,y):(x,y+1):(x+1,y+1)$, etc.


   The construction will actually control the width of the square only to within an additive logarithmic factor by bring together blocks of width and length $\Theta(\log n)$; standard techniques can be used to make the square precisely $n \times n$.
   For instance, we could add $O(\log n)$ total filler tiles to the leftmost and bottommost blocks, while adding only $O(\log^2 n)$ to the assembly depth and $O(\log \log n)$ to the tile complexity since such filler tiles could be assembled from a counter that counts to $\log n$ using $O(\log \log n)$ tile types.
   For simplicity we describe the desired width $n$ as the number of blocks instead of the desired dimensions of the square and omit the details of this last step of filling in the logarithmic gap.

   Figure~\ref{fig:two-handed-square-high-level} outlines the construction of a square when the number of blocks $n$ is a power of two.
   Figure~\ref{fig:two-handed-square-non-power-of-2} shows how to modify the blocks so that some of them are double in width, double in height, or both, to achieve a total square width that is an arbitrary positive integer.
   Each block contains the same $O(\frac{\log n}{\log \log n})$ tile types that encode $n$, and as the block assembles it randomly chooses $x$ and $y$-coordinates, which represent an index in the square.
   This random choice is implemented through competition between tile types that share the same ``input'' glues but represent different bits of $x$ or $y$. %\footnote{A curious feature of hierarchical TAS's is that the TAS can remain directed despite this nondeterministic competition, whereas it cannot happen in any directed seeded TAS.}
   These are used to determine the block's own size and to determine what series of bumps and dents to place on its perimeter to enforce that the only blocks that can bind are adjacent in Figure~\ref{fig:two-handed-square-high-level}.
   The coordinates are also used to determine where to place strength-1 glues. The same strength-1 glue is used uniformly throughout Figure~\ref{fig:two-handed-square-high-level}.
   The bumps and dents ensure that no two blocks can attach unless they are adjacent in the figure.

   The growth of an individual block is shown in Figure~\ref{fig:two-handed-square-block}.
   We describe the assembly as if it grows only by single-tile accretion.
   There are some strength-2 glues so this is not completely accurate, but the growth of the block is ``polyomino-safe'', to borrow a term of Winfree~\cite{Winfree06}.
   By design, no assembly larger than four can form except by attachment to the growing block, and even if these assemblies attach at once to the block rather than by single-tile accretion, the correct operation of the block growth is unaffected.
   This is due to the fact that all strength-2 glues are ``one-to-one''; no strength-2 glue is shared as an ``output'' (in the direction of growth in the seeded model) by two different tile types.
   This implies that no partial assembly occurring away from the main ``seeded'' assembly can grow ``backward'' and place an incorrect tile.

   To form a square of size $n \times n$ ``units'' (where a unit is $O(\log n)$, the width and height of a small block), we choose the largest power of two $2^k \leq n$ and assemble exactly $2^k \times 2^k$ different types of blocks, doubling the width (resp. height) of the first $n-2^k$ of them in the $x$-direction (resp. $y$-direction), as in Figure~\ref{fig:two-handed-square-non-power-of-2}.
   The orange (medium darkness in gray-scale) tile types in Figure~\ref{fig:two-handed-square-block} are the only non-constant set of tile types.
   Borrowing a technique from~\cite{AdChGoHu01}, we will represent $n$ in base $b$, where $b \approx \log n / \log \log n$, using $\approx \log n / \log \log n$ unique tile types, and we use a constant number of tile types to convert $n-2^k$ to binary and accomplish all the other tasks needed to assemble the block.

   Choose $b=2^m$ to be a power of two such that $\log n / \log \log n \leq b < 2 \log n / \log \log n.$
   Each digit in base $b$ can represent $m$ bits of $n-2^k$.
   $n-2^k$ is encoded in exactly $m \cdot \ceil{\frac{k}{m}} = O(\frac{\log n}{\log \log n})$ base-$b$ digits.
   The blue (dark in gray-scale) tile types in Figure~\ref{fig:two-handed-square-block} convert $n-2^k$ from base $b$ to binary and at the same time represent $n-2^k$ with its ``bit-quadrupled'' version (e.g., $0110 \mapsto 0000111111110000$), since each bit along the edge will eventually require width four to make room to place the bumps properly.\footnote{The bumps cannot simply be placed with strength-2 glues above a width-1 or even width-2 representation of a bit in the obvious way, otherwise there would be nothing to force that the bumps are present before the inter-block strength-1 glues.  If the bumps are allowed to grow in parallel with the rest of the assembly then they may not complete fast enough.  Width four is required to create a ``linear assembly path'' for the bumps and dents tiles to follow, ensuring that growth of the block continues only once the path is complete.}
   %At the same time $n-2^k$ is converted to binary, every fourth position along the row, there is a nondeterministic competition among four tile types to determine a bit of $x$ and a bit of $y$.
   The counterclockwise order of growth ensures that if not all of the bumps and dents are formed, then at least one of the four strength-1 glues necessary for an attachment event to occur is not yet present in one of the blocks.
   To ensure that the TAS is directed, we do not include base-conversion tiles for any digit $d \in \{0,1,\ldots,b-1\}$ that does not appear in the base-$b$ expansion of $n-2^k$, otherwise those tiles will form unused terminal assemblies.
   Each glue in a tile type representing a bit is ``marked'' indicating whether it is the most significant bit, least significant bit, or interior bit, as well as being marked with its relative position among the four copies of the bit.

   Once $n-2^k$ is converted to binary, we use nondeterministic attachment of tiles to the north of this value to randomly guess $2k$ bits that represent the $x$- and $y$-coordinates of the block, meaning the binary numbers represented on the top and right, respectively, of each block in Figure~\ref{fig:two-handed-square-high-level}.
   To be precise, we must actually choose each of $x$ and $y$ to be a random bit string that is not all 1's, since each represents a connection between two blocks, of which there are $2^k-1$ along each dimension.
   It is straightforward to encode into the tile types the logic that if the first $k$ bits were 1, then the final bit must be 0.
   A number of additional computations are done on these values (some computations are possible to do as the values are guessed).
   The results of these computations will be stored in the rightmost tile type and propagated to all subsequent tile types.
   First, each of $x$ and $y$ is compared to $n-2^k$ to determine how large to make each dimension of the block.
   In the example of Figure~\ref{fig:two-handed-square-block}, $y < n-2^k$ and $x \geq n-2^k$, so the block is one ``unit'' wide and two ``units'' high.
   Also, the binary expansions of $x$ and $y$ are themselves compared to determine where to place strength-1 glues.
   After $x$ and $y$ are determined, to place bumps and dents on the left and bottom of the block, the values $x-1$ and $y-1$ must be computed, which requires assembling from least significant to most significant, so this is delayed until after the first 90-degree rotation shown in Figure~\ref{fig:two-handed-square-block}.
   Once these values are computed, they are also used to determine placement of glues.
   The entire block is created by rotating either counter-clockwise (in the case of $x$ even, as shown in the bottom right of Figure~\ref{fig:two-handed-square-block}) or clockwise (in the case of $x$ odd, not shown but the exact mirror image of the bottom right of Figure~\ref{fig:two-handed-square-block}), placing bumps and dents and single-strength glues.
   The glues are placed in the order shown by the rotations, so that the last glue to be (potentially) placed is the top east-facing glue in the case of $x$ even, or the top west-facing glue in the case of $x$ odd.


   By inspection of Figure~\ref{fig:two-handed-square-high-level}, it is routine to verify that the following rules can be used to determine placement of strength-1 glues.
   If $x$ is even, then place two single-strength glues on the right edge.
   If $x$ is odd, then place two single-strength glues on the left edge.
   For a natural number $n$, define $t(n)$ to be the number of trailing 1's in $n$'s binary expansion.
   If $t(x) \geq t(y)$, then place exactly one strength-1 glue on the top edge.
   If $t(x) \geq t(y-1)$, then place exactly one strength-1 glue on the bottom edge.
   If $t(x-1) \leq t(y)+1$ and $x$ is even, then place exactly one strength-1 glue on the left edge.
   If $t(x) \leq t(y)+1$ and $x$ is odd, then place exactly one strength-1 glue on the right edge.

   Each of these computations (for placement of glues and for determining block dimensions) can be computed by a deterministic finite automaton whose input symbols represent tuples of bits from $n-2^k$, $x$, $x-1$, $y-1$, and $y$.
   These automata can then be combined in a product construction and embedded into the tile types that accrete in the row above $n-2^k$ if only $x$ and $y$ are needed, and embedded into tile types that are placed after the first rotation if $x-1$ or $y-1$ is needed.
   Since the decision for placing glue on the top edge requires only $x$ and $y$, this ensures that the decision for each glue placement can be made before the region containing the potential glue site is assembled.

   As shown in Figure~\ref{fig:two-handed-square-block}, some padding with filler tiles is necessary to make the block a perfect rectangle.
   Also, some padding is needed in the case of a doubling of height or width, to ensure that the resulting assembly has height or width precisely twice that of the non-doubled version.
}

\opt{normal}{
    \begin{proof}
    \ProofParallelSquare
    \end{proof}
}


















